Probing Pre-trained Auto-regressive Language Models for Named Entity Typing and Recognition

Despite impressive results of language models for named entity recognition (NER), their generalization to varied textual genres, a growing entity type set, and new entities remains a challenge. Collecting thousands of annotations in each new case for training or fine-tuning is expensive and time-consuming. In contrast, humans can easily identify named entities given some simple instructions. Inspired by this, we challenge the reliance on large datasets and study pre-trained language models for NER in a meta-learning setup. First, we test named entity typing (NET) in a zero-shot transfer scenario. Then, we perform NER by giving few examples at inference. We propose a method to select seen and rare / unseen names when having access only to the pre-trained model and report results on these groups. The results show: auto-regressive language models as meta-learners can perform NET and NER fairly well especially for regular or seen names; name irregularity when often present for a certain entity type can become an effective exploitable cue; names with words foreign to the model have the most negative impact on results; the model seems to rely more on name than context cues in few-shot NER.

==> abstract_lrec.tex <==
Multiple works have proposed to probe language models (LMs) for generalization in named entity (NE) typing (NET) and recognition (NER).
However, little has been done in this direction for auto-regressive models despite their popularity and potential to express a wide variety of NLP tasks in the same unified format.
We propose a new methodology to probe auto-regressive LMs for NET and NER generalization, which draws inspiration from human linguistic behavior, by resorting to meta-learning.
We study NEs of various types individually by designing a zero-shot transfer strategy for NET.
Then, we probe the model for NER by providing a few examples at inference.
We introduce a novel procedure to assess the model's memorization of NEs and report the memorization's impact on the results.
Our findings show that: 
1) pre-trained auto-regressive LMs, without any fine-tuning for NET or NER, perform the tasks fairly well;
%, so the pre-training impact should always be explicitly considered; 
2) name irregularity when common for a NE type could be an effective exploitable cue;
3) the model seems to rely more on NE than contextual cues in few-shot NER;
4) NEs with words absent during LM pre-training are very challenging for both NET and NER.
